2-Colorable Perfect Matching is NP-complete in 2-Connected 3-Regular Planar Graphs

The 2-colorable perfect matching problem asks whether a graph can be colored with two colors so that each node has exactly one neighbor with the same color as itself. We prove that this problem is NP-complete, even when restricted to 2-connected 3-regular planar graphs. In 1978, Schaefer proved that this problem is NP-complete in general graphs, and claimed without proof that the same result holds when restricted to 3-regular planar graphs. Thus we fill in the missing proof of this claim, while simultaneously strengthening to 2-connected graphs (which implies existence of a perfect matching). We also prove NP-completeness of $k$-colorable perfect matching, for any fixed $k \geq 2$.

==> conclusion.tex <==
In this paper, we have filled the gap left in Schaefer's \textit{The Complexity of Satisfiability Problems} by proving that 2-colorable perfect matching problem is NP-complete even when the graph is restricted to be planar and 3-regular. We have also extended the result by restricting the graph to be 2-connected as well. This result could introduce a new class of complexity problem to bridge the gap between our NP-complete result and the existing polynomial algorithm to find perfect matching in 2-connected 3-regular graphs. Some possible variants are coloring when some nodes are already paired, coloring when the perfect matching is not required, and/or the approximation version.

Apart from that, we have also extended the 2-colorable result by exploring the case with more colors. We proved that the $k$-colorable perfect matching problem still remains NP-complete for any $k > 2$. Similar to our main result, it would be interesting to restrict the graph to be 3-regular, 2-connected, or planar as well. A potential solution would be to modify the gadgets that are used in our main result to work on $k$ colors instead. Combining this with our new gadget, we will be able to reduce from our main result. However, with colors more than 2, it is more difficult to force the coloring. Thus, a reasonable next step would be to restrict the properties of a graph one at a time and to try with just three colors.
